Improving Predictability of User-Affecting Metrics to Support Anomaly Detection in Cloud Services

Anomaly detection systems aim to detect and report attacks or unexpected behavior in networked systems. Previous work has shown that anomalies have an impact on system performance, and that performance signatures can be effectively used for implementing an IDS. In this paper, we present an analytical and an experimental study on the trade-off between anomaly detection based on performance signatures and system scalability. The proposed approach combines analytical modeling and load testing to find optimal configurations for the signature-based IDS. We apply a heavy-tail bi-modal modeling approach, where "long" jobs represent large resource consuming transactions, e.g., generated by DDoS attacks; the model was parametrized using results obtained from controlled experiments. For performance purposes, mean response time is the key metric to be minimized, whereas for security purposes, response time variance and classification accuracy must be taken into account. The key insights from our analysis are: (i) there is an optimal number of servers which minimizes the response time variance, (ii) the sweet-spot number of servers that minimizes response time variance and maximizes classification accuracy is typically smaller than or equal to the one that minimizes mean response time. Therefore, for security purposes, it may be worth slightly sacrificing performance to increase classification accuracy.

==> 400_biography.tex <==
%\newpage
%\clearpage
\phantomsection
% Vilc Rufino
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in, clip, keepaspectratio] {img/improve/bio/vilc_bw.png}}] 
    {Vilc Queupe Rufino} 
    (S'19) 
    received the B.S. degree in computer engineering from Federal University of Espírito Santo, in 1999, and the M.S. degree in Computer Science from University of São Paulo, in 2009. He is currently pursuing his Ph.D. at the Federal University of Rio de Janeiro (UFRJ). He has been in the Navy Corps of Engineers as technical officer since 2000. His interests include modeling and analysis of  systems, with  focus on security.  
\end{IEEEbiography}

% Mateus Nogueira
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in, clip, keepaspectratio] {img/improve/bio/mateus_nogueira_bw.png}}]
    {Mateus Schulz Nogueira} 
    received the B.S. degree in Computer Science from Federal University of Rio de Janeiro (UFRJ), in 2019. He is currently pursuing his M.Sc. in Informatics, also at UFRJ.  His interests include modeling and analysis of  systems, with  focus on machine learning.
\end{IEEEbiography}

% Alberto Avritzer
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/improve/bio/alberto_bw.png}}] 
    {Alberto Avritzer} 
    is the founder and CEO of eSulabSolutions Inc, the preferred source for methods for scalability assessment of mission-critical systems in the telecom and banking domains. He led the automated performance testing and analysis of New York subway public announcement and customer information system (PA/CIS), where he was responsible for the certification of system scalability to support 550 stations. Alberto received a Ph.D. in Computer Science from the University of California, Los Angeles, an M.Sc. in Computer Science for the Federal University of Minas Gerais, Brazil, and the B.Sc. in Computer Engineering from the Technion, Israel Institute of Technology. He served as Lead Performance Engineer at Sonatype, MD, and as a Senior Member of the Technical Staff in the Software Engineering Department at Siemens Corporate Research, Princeton, New Jersey. Before moving to Siemens Corporate Research, he spent 13 years at AT\&T Bell Laboratories, where he developed tools and techniques for performance testing and analysis. He spent the summer of 1987 at IBM Research, at Yorktown Heights.  His research interests are in software engineering, particularly software testing, monitoring and rejuvenation of smoothly degrading systems, and metrics to assess software architecture, and he has published over 70 papers in journals and refereed conference proceedings in those areas.
    He is a Senior Member of ACM. He has presented several tutorials at international conferences such as LADC, IEEE ISSRE and ACM ICPE. 
\end{IEEEbiography}

%Daniel Sadoc
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in, clip, keepaspectratio]{img/improve/bio/daniel_bw.png}}]
    {Daniel Sadoc Menasch\'e} 
    received the Ph.D. degree in Computer Science from the University of Massachusetts, Amherst, in 2011. Currently, he is an Associate Professor with the Computer Science Department, Federal University of Rio de Janeiro, Rio de Janeiro, Brazil. His interests are in modeling, analysis, security and performance evaluation of computer systems, being a recipient of best paper awards at GLOBECOM 2007, CoNEXT 2009, INFOCOM 2013 and ICGSE 2015.  He is currently an affiliated member of the Brazilian Academy of Sciences.
\end{IEEEbiography}

% Barbara Russo
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/improve/bio/barbara_russo_bw.png}}]
    {Barbara Russo} is a full professor at the Faculty of Computer Science of the Free University of Bozen-Bolzano, Italy. 
    She received the Ph.D. degree (with distinciton) in mathematics from the University of Trento, Italy.
   She was  visiting researcher at the Max-Plank Institute fuer Mathematik, Bonn, Germany. Her research interests include	machine learning for the identification and prediction of anomalies, bugs, and vulnerabilities of dependable systems;
	data mining to monitor, understand, predict system maintenance; continuous automated testing of modern software systems.
\end{IEEEbiography}

% Andrea Janes
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/improve/bio/andrea_janes_bw.png}}]
    {Andrea Janes}   
    is a researcher with a fixed-term contract at the Free University of Bolzano-Bozen (Italy). His research interests include Lean and Agile software development, value-based software engineering, and empirical software engineering. He received his Master’s degree in business informatics from the Technical University of Vienna, Austria and received a doctorate in computer science (with distinction) from the University of Klagenfurt (Austria). Since 2017 he is also involved in technology transfer projects within the Smart Data Factory at the NOI Techpark Sdtirol/Alto Adige in Bolzano.
\end{IEEEbiography}

% Vincenzo Ferme
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/improve/bio/vincenzo_ferme_bw.png}}]
    {Vincenzo Ferme} 
    is a Cloud and DevOps Expert at Kiratech Switzerland and a Ph.D. Candidate at the University of Lugano (USI), Switzerland. He has received his Bachelor’s degree from University of Federico II, Naples (Italy) and his Master’s degree from the University Milano-Bicocca, Milan (Italy). Before starting his Ph.D., he was a Software Engineer and Java Developer at Connexun s.r.l. for one year. Vincenzo’s research is focused on the automation of Performance Testing in DevOps.
\end{IEEEbiography}

% Andre Van Hoorn
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/improve/bio/andre_van-hoorn_bw.png}}]
    {Andre Van Hoorn} 
    is a senior researcher with the Institute of Software Technology at the University of Stuttgart, Germany. He received his Ph.D. degree (with distinction) from Kiel University, Germany and his Master’s degree from the University of Oldenburg, Germany. His research focuses on designing, operating, and evolving trustworthy distributed software systems, focusing on quality attributes such as performance, reliability, and resilience. Currently, André investigates challenges and opportunities in the context of continuous software engineering and DevOps.
\end{IEEEbiography}

% Henning Schulz
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/improve/bio/henning_schulz_bw.png}}]
    {Henning Schulz}  
    is a consultant for Application Performance Management (APM) at Novatec Consulting GmbH, Germany, and an external Ph.D. candidate at the Reliable Software System’s Group of the University of Stuttgart (Institute of Software Technology), Germany. He received his Master’s degree in Informatics from the Karlsruhe Institute of Technology, Germany. His research focus is workload characterization and representative load testing in continuous software engineering.
\end{IEEEbiography}


% Cabral Lima
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/improve/bio/cabral_bw.png}}]
    {Cabral Lima} 
    received the Ph.D. degree in computer science from Université Pierre et Marie Currie (Paris 6), France.
    Currently, he is a Full Professor with the Computer Science Department, Federal University of Rio de Janeiro, Rio de Janeiro, Brazil. His interests are modeling and analysis of computer system, optimization and intelligent robotics. Dr. Cabral was recipient of best paper award at ICONS 2014 and Meritorious Award at International Institute for Advanced Studies in System Research and Cybernetics, Germany, 2002.
\end{IEEEbiography}

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

